AmbiFC: Fact-Checking Ambiguous Claims with Evidence

Automated fact-checking systems verify claims against evidence to predict their veracity. In real-world scenarios, the retrieved evidence may not unambiguously support or refute the claim and yield conflicting but valid interpretations. Existing fact-checking datasets assume that the models developed with them predict a single veracity label for each claim, thus discouraging the handling of such ambiguity. To address this issue we present AmbiFC, a fact-checking dataset with 10k claims derived from real-world information needs. It contains fine-grained evidence annotations of 50k passages from 5k Wikipedia pages. We analyze the disagreements arising from ambiguity when comparing claims against evidence in AmbiFC, observing a strong correlation of annotator disagreement with linguistic phenomena such as underspecification and probabilistic reasoning. We develop models for predicting veracity handling this ambiguity via soft labels and find that a pipeline that learns the label distribution for sentence-level evidence selection and veracity prediction yields the best performance. We compare models trained on different subsets of AmbiFC and show that models trained on the ambiguous instances perform better when faced with the identified linguistic phenomena.

==> figures/claim-rewriting.tex <==
\begin{figure}[]
\centering
\begin{tabular}{|l|}
\hline

\textbf{BoolQ query:}                                                                           \\
Is it illegal in Illinois to record a conversation?                                                        \\
\textbf{Generated Claim:}                                                                                   \\
It is illegal in Illinois to record a conversation.                                                    \\

\hline
\end{tabular}
\caption{Generating dataset instances by rewriting queries from BoolQ as claims and extracting sentence-level evidence from Wikipedia.}
\label{fig:annotation-example}
\end{figure}

==> figures/running-example-v2.tex <==
\begin{figure}
\small
    \centering
    \includegraphics[width=0.9\linewidth]{pictures/intro-example-v2png.png}
    \caption{The instance of claim and evidence from \datasetname{} is ambiguous due to underspecification.}
    \label{fig:running-example}
\end{figure}

==> figures/runnning-example.tex <==
\begin{figure}[]
\centering
\begin{tabular}{|l|}
\hline

    \textbf{Claim}: \textit{It is illegal in Illinois to record a con-}\\ \textit{versation.} \\
    \textbf{Evidence}: \textit{Illinois made it a crime to use an} \\ \textit{"eavesdropping device" to overhear or record} \\ \textit{a phone call or conversation without the consent}\\ \textit{of all parties to the conversation.}\\
\hline

\end{tabular}
    \caption{An example claim and evidence pair from the dataset presented in this paper, which is ambiguous due to underspecification.}
    \label{fig:running_example}
\end{figure}

==> tables/aggregated-performance-on-uncertain.tex <==
\begin{table*}[ht]
\centering
\small
    \centering
    \begin{tabular}{lcc | c c c | c c | c}
    \toprule    
    \multicolumn{3}{c|}{\textit{Model}} & 
    \multicolumn{3}{c|}{\textit{T2 (F1)}} & 
    \multicolumn{2}{c|}{\textit{T2}} & 
    \textit{T1+T2} \\
    
    \midrule
    \textbf{Train} & \textbf{T1} & \textbf{T2} & \textbf{Supp.} & \textbf{Ref.} & \textbf{Neut.} & \textbf{Acc.} & \textbf{F1}  & \textbf{w-Acc.}\\
    \midrule

    % XX \tiny{$\pm XX$}& XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$}& XX \tiny{$\pm XX$}\\   
    
    -- & \textit{oracle} & \textsc{Majority} &72.7 & 71.1& 4.0 & 59.0 & 49.3& 59.0\\
    -- & \textit{oracle} & \textsc{LastSent} & 71.4 & 69.4 &  4.0& 57.8 &48.2& 57.8\\
    \midrule

    \datacertain{} & \textit{oracle} & \textsc{PSingle} & 73.6 \tiny{$\pm 0.3$}& 65.3 \tiny{$\pm 1.4$} & 67.5 \tiny{$\pm 0.6$} & 69.7 \tiny{$\pm 0.2$} & 68.8 \tiny{$\pm 0.4$}& 69.7 \tiny{$\pm 0.2$}\\  
    \datauncertainfp{} & \textit{oracle} & \textsc{PSingle} & 75.7 \tiny{$\pm 0.5$}& \textbf{69.0} \tiny{$\pm 0.8$} & 65.9 \tiny{$\pm 0.4$} & 70.8 \tiny{$\pm 0.4$} & 70.2 \tiny{$\pm 0.4$}& 70.8 \tiny{$\pm 0.4$}\\    
    \datauncertain{} & \textit{oracle} & \textsc{PSingle} & 75.1 \tiny{$\pm 0.6$}& 67.1 \tiny{$\pm 2.3$} & \textbf{69.7} \tiny{$\pm 0.3$} & 71.3 \tiny{$\pm 0.6$} & 70.6 \tiny{$\pm 0.9$}& 71.3 \tiny{$\pm 0.6$}\\    
    \datasetname{} & \textit{oracle} & \textsc{PSingle} & \textbf{76.2} \tiny{$\pm 0.4$}& 68.9 \tiny{$\pm 0.9$} & 67.6 \tiny{$\pm 0.3$} & \textbf{71.6} \tiny{$\pm 0.3$} & \textbf{70.9} \tiny{$\pm 0.4$}& \textbf{71.6} \tiny{$\pm 0.3$}\\    
    \midrule

    \datacertain{} & binary & \textsc{PSingle} & 66.7 \tiny{$\pm 1.0$}& 56.7 \tiny{$\pm 1.3$} & 66.9 \tiny{$\pm 0.2$} & 64.9 \tiny{$\pm 0.4$} & 63.4 \tiny{$\pm 0.6$}& 30.7 \tiny{$\pm 1.3$}\\  
    \datauncertainfp{} & binary & \textsc{PSingle} & 73.0 \tiny{$\pm 0.5$}& \textbf{65.5} \tiny{$\pm 0.5$} & 63.1 \tiny{$\pm 1.6$} & 67.8 \tiny{$\pm 0.4$} & 67.2 \tiny{$\pm 0.5$}& \textbf{44.3} \tiny{$\pm 0.6$}\\    
    \datauncertain{} & binary & \textsc{PSingle} & 68.1 \tiny{$\pm 1.1$}& 60.5\tiny{$\pm 3.2$} & \textbf{67.6} \tiny{$\pm 0.6$} & 66.4 \tiny{$\pm 1.0$} & 65.4 \tiny{$\pm 1.4$}& 35.1 \tiny{$\pm 1.3$}\\    
    \datasetname{} & binary & \textsc{PSingle} & \textbf{73.2} \tiny{$\pm 0.6$}& 65.2 \tiny{$\pm 1.4$} & 67.0 \tiny{$\pm 0.8$} & \textbf{69.1} \tiny{$\pm 0.4$} & \textbf{68.5} \tiny{$\pm 0.6$}& 42.0 \tiny{$\pm 0.5$}\\   
    \midrule

    \datacertain{} & \multicolumn{2}{c|}{\textsc{FSingle}} & 69.2 \tiny{$\pm 1.6$}& 59.5 \tiny{$\pm 3.2$} & 67.3 \tiny{$\pm 0.3$} & 66.6 \tiny{$\pm 1.1$} & 65.4 \tiny{$\pm 1.5$}& --\\ 
    \datauncertainfp{} & \multicolumn{2}{c|}{\textsc{FSingle}} & 72.9 \tiny{$\pm 0.3$}& 65.8 \tiny{$\pm 1.2$} & 62.9 \tiny{$\pm 0.8$} & 67.8 \tiny{$\pm 0.3$} & 67.2 \tiny{$\pm 0.5$}& --\\    
    \datauncertain{} &\multicolumn{2}{c|}{\textsc{FSingle}} & 69.6 \tiny{$\pm 2.7$}& 62.8 \tiny{$\pm 3.2$} & \textbf{68.2} \tiny{$\pm 0.5$} & 67.7 \tiny{$\pm 1.6$} & 66.8 \tiny{$\pm 2.0$}& --\\    
    \datasetname{} & \multicolumn{2}{c|}{\textsc{FSingle}} & \textbf{73.4} \tiny{$\pm 1.0$}& \textbf{65.9} \tiny{$\pm 1.1$} & 66.7 \tiny{$\pm 0.7$} &\textbf{69.3} \tiny{$\pm 0.4$} & \textbf{68.7} \tiny{$\pm 0.4$}& --\\  
%    -- & \textit{oracle} & \textsc{ConfSent} & XX \tiny{$\pm XX$}& XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$}& XX \tiny{$\pm XX$}\\    
        
       \bottomrule
    \end{tabular}
    \caption{Evaluation on aggregated labels on the \datauncertainfp{}. Just because it may be interesting. Will probably not be included in the final version because we use soft-label evaluation there. }
    \label{tbl:results-aggregated-label-uncertain}
\end{table*}{}

==> tables/error_analysis.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l | c }
    Inference Type & DistCS  \\
    \toprule
    {Implicature} & 73.40\\
    {Presupposition} & 73.75\\
    {Coreference} & 79.04\\
    {Vagueness} & 75.33\\
    {Underspecification} & 80.49\\
    {Probabilistic reasoning} & 75.51\\
      \bottomrule
    \end{tabular}
    \caption{Results of the best performing model (Annotation Distillation) as measured by the strictest metric (DistCS) per inference type.}
    \label{tbl:error_analysis}
\end{table}


==> tables/justification-drop-neutral-relevant.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l | c c}
       & \multicolumn{2}{c}{\textit{Sampled 2$\times$ neutral and}} \\
        \textbf{Subset} & \textbf{not relevant} & \textbf{relevant} \\
        \toprule
        certain& 2.2 \% \tiny{$\pm$0.1} & 0.0 \% \tiny{$\pm$0.0}\\
        uncertain &0.6 \% \tiny{$\pm$0.0}& 20.9 \% \tiny{$\pm$0.2}\\
        all & 0.9 \% \tiny{$\pm$0.0}& 16.8 \% \tiny{$\pm$0.1}\\
        \bottomrule
        
    \end{tabular}
    \caption{Likelihood of misclassifying a non-neutral sample as neutral with only two seen annotations.}
    \label{tbl:stochastic-simulation-dataset-neutral-relevant}
\end{table}

==> tables/main_results_aggregated_labels.tex <==
\begin{table*}[ht]
\centering
\small
    \centering
    \begin{tabular}{lcc | c c :c| c :c}
    \toprule
    \multicolumn{3}{c|}{\textit{}} & \multicolumn{3}{c|}{\datacertain{}} & \multicolumn{2}{c}{\datacertainfp{}} \\
    
    \multicolumn{3}{c|}{\textit{Model}} & 
    \multicolumn{2}{c|}{\textit{T2}} & 
    \textit{T1+T2} & 
    \textit{T2} & 
    \textit{T1+T2} \\
    
    \midrule
    \textbf{Train} & \textbf{T1} & \textbf{T2} & \textbf{Acc.} & \textbf{F1} & \textbf{w-Acc.} & \textbf{Acc.} & \textbf{w-Acc.}\\
    \midrule

    % XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX  \tiny{$\pm XX$} \\
    
    -- & \textit{oracle} & \textsc{Majority} & \textit{98.5} & \textit{96.7} & \textit{98.5} & \textit{94.4}  & \textit{94.4} \\
    -- & \textit{oracle} & \textsc{LastSent} & \textit{98.5} & \textit{96.7} & \textit{98.5} & \textit{94.4}  & \textit{94.4} \\
    \midrule

    \datacertain{} & \textit{oracle} & \textsc{Single} & 97.1 \tiny{$\pm 0.1$} & 93.0 \tiny{$\pm 0.2$} & 97.1 \tiny{$\pm 0.1$} & 89.3 \tiny{$\pm 0.5$} & 89.3  \tiny{$\pm 0.5$} \\
    \datauncertainfp{} & \textit{oracle} & \textsc{Single} & 97.7 \tiny{$\pm 0.1$} & 94.5 \tiny{$\pm 0.2$} & 97.7 \tiny{$\pm 0.1$} & 91.5 \tiny{$\pm 0.3$} & 91.5  \tiny{$\pm 0.3$} \\
    \datauncertain{} & \textit{oracle} & \textsc{Single} & 97.4 \tiny{$\pm 0.2$} & 93.7 \tiny{$\pm 0.5$} & 97.4 \tiny{$\pm 0.2$} & 90.2 \tiny{$\pm 0.8$} & 90.2  \tiny{$\pm 0.2$} \\
    \datasetname{} & \textit{oracle} & \textsc{Single} & 97.7 \tiny{$\pm 0.2$} & 94.4 \tiny{$\pm 0.4$} & 97.7 \tiny{$\pm 0.2$} & 91.5 \tiny{$\pm 0.6$} & 91.5  \tiny{$\pm 0.6$} \\
    \midrule
    
    \datasetname{} & stance & \textsc{Majority} & 89.1 \tiny{$\pm 2.2$} & 79.2 \tiny{$\pm 4.9$} & 82.9 \tiny{$\pm 2.2$} & 79.7 \tiny{$\pm 10.9$} & 56.7  \tiny{$\pm 9.9$} \\
    \datasetname{} & stance & \textsc{LastSent} & 89.0 \tiny{$\pm 2.4$} & 78.9 \tiny{$\pm 4.6$} & 82.8 \tiny{$\pm 2.4$} & 79.1 \tiny{$\pm 10.2$} & 56.4  \tiny{$\pm 9.4$} \\
    \datasetname{} & stance & \textsc{ConfSent} & 89.1 \tiny{$\pm 2.2$} & 78.9 \tiny{$\pm 4.9$} & 82.9 \tiny{$\pm 2.3$} & 79.5 \tiny{$\pm 10.9$} & 56.5  \tiny{$\pm 9.7$} \\

    \datacertain{} & stance & \textsc{Majority} & 91.4 \tiny{$\pm 0.6$} & 83.7 \tiny{$\pm 1.4$} & \textbf{85.2} \tiny{$\pm 0.5$} & 80.5 \tiny{$\pm 5.7$} & 57.5  \tiny{$\pm 5.2$} \\
    \datacertain{} & stance & \textsc{LastSent} & 91.2 \tiny{$\pm 0.5$} & 83.3 \tiny{$\pm 1.2$} & 85.1 \tiny{$\pm 0.5$} & 80.0 \tiny{$\pm 5.5$} & 57.2  \tiny{$\pm 5.2$} \\
    \datacertain{} & stance & \textsc{ConfSent} & \textbf{91.5} \tiny{$\pm 0.6$} & \textbf{83.9} \tiny{$\pm 1.4$} & \textbf{85.2} \tiny{$\pm 0.5$} & \textbf{80.8} \tiny{$\pm 5.7$} & \textbf{57.6}  \tiny{$\pm 5.2$} \\
    \midrule

    
% XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX \tiny{$\pm XX$} & XX  \tiny{$\pm XX$} \\


    \datacertain{} & binary & \textsc{Single} & 93.9 \tiny{$\pm 0.2$} & 87.9 \tiny{$\pm 0.5$} & \textbf{83.6} \tiny{$\pm 1.0$} & 83.6 \tiny{$\pm 1.1$} & 62.5  \tiny{$\pm 0.6$} \\
    \datauncertainfp{} & binary & \textsc{Single} & 92.1 \tiny{$\pm 0.7$} & 86.1 \tiny{$\pm 1.0$} & 58.9 \tiny{$\pm 3.5$} & \textbf{89.8} \tiny{$\pm 0.8$} & \textbf{68.2}  \tiny{$\pm 0.7$} \\
    \datauncertain{} & binary & \textsc{Single} & \textbf{94.2} \tiny{$\pm 0.2$} & 88.6 \tiny{$\pm 0.4$} & 82.7 \tiny{$\pm 0.7$} & 84.7 \tiny{$\pm 1.0$} & 63.4  \tiny{$\pm 0.9$} \\
    \datasetname{} & binary & \textsc{Single} & 94.1 \tiny{$\pm 0.2$} & \textbf{88.9} \tiny{$\pm 0.4$} & 77.0 \tiny{$\pm 1.5$} & 89.1 \tiny{$\pm 0.5$} & 67.7  \tiny{$\pm 0.3$} \\
    \midrule

    \datacertain{} & \multicolumn{2}{c|}{\textsc{Single}} & 94.1 \tiny{$\pm 0.3$} & 88.3 \tiny{$\pm 0.8$} & -- & 85.5 \tiny{$\pm 1.7$} & -- \\
    \datauncertainfp{} & \multicolumn{2}{c|}{\textsc{Single}} & 91.9 \tiny{$\pm 0.4$} & 85.7 \tiny{$\pm 0.5$} & -- & 90.0 \tiny{$\pm 0.8$} & -- \\
    \datauncertain{} & \multicolumn{2}{c|}{\textsc{Single}} & \textbf{94.4} \tiny{$\pm 0.3$} & 89.1 \tiny{$\pm 0.6$} & -- & 86.3 \tiny{$\pm 2.7$} & -- \\
    \datasetname{} & \multicolumn{2}{c|}{\textsc{Single}} & \textbf{94.4} \tiny{$\pm 0.2$} & \textbf{89.4} \tiny{$\pm 0.4$} & -- & \textbf{90.1} \tiny{$\pm 0.7$} & -- \\


        
       \bottomrule
    \end{tabular}
    \caption{TBA. Possibly add some pretraining? But we can also have a separate Pretraining table simply with the best result from here. Results are Accuracy and Macro F1-score (T1), and evidence-weighted accuracy (T1+T2). \textbf{Todo:} I now report the reuslts on the two subsets of \datasetname{} separately. May reduce. Results arew averaged over 3 seeds. We do not report macro F1 on \datacertainfp{} because it almost entirely consists of non-neutral samples. \textbf{Todo:} remove unrequired.}
    \label{tbl:main-results-aggregated-label_old}
\end{table*}{}
